Ophthalmic Biomarker Detection: Highlights from the IEEE Video and Image Processing Cup 2023 Student Competition

The VIP Cup offers a unique experience to undergraduates, allowing students to work together to solve challenging, real-world problems with video and image processing techniques. In this iteration of the VIP Cup, we challenged students to balance personalization and generalization when performing biomarker detection in 3D optical coherence tomography (OCT) images. Balancing personalization and generalization is an important challenge to tackle, as the variation within OCT scans of patients between visits can be minimal while the difference in manifestation of the same disease across different patients may be substantial. The domain difference between OCT scans can arise due to pathology manifestation across patients, clinical labels, and the visit along the treatment process when the scan is taken. Hence, we provided a multimodal OCT dataset to allow teams to effectively target this challenge. Overall, this competition gave undergraduates an opportunity to learn about how artificial intelligence can be a powerful tool for the medical field, as well as the unique challenges one faces when applying machine learning to biomedical data.

==> Sections/2_tasks_resources_eval.tex <==
The 2023 VIP Cup competition consists of two distinct phases, each with unique challenges and assessment criteria. In this section, we provide an overview of the tasks teams are challenged to complete, along with the provided resources and the criteria teams are evaluated on.

\subsection{VIP Cup Tasks}

The competition takes place across two phases, which aim at testing teams' approaches to both the generalization and personalization challenges present within ophthalmology data. Throughout this section, we describe the specific tasks present within each competition phase.

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{Modality} & \textbf{Per Visit} & \textbf{Per Eye} & \textbf{Train Total} & \textbf{Phase 1 Test Set} & \textbf{Phase 2 Test Set} \\ \hline
OCT               & 49                 & $N_{p}*49$            & 78189                & 3871                      & 250                       \\ \hline
Clinical          & 4                  & $N_{p}*4$             & 5082                 & 320                       & 250                       \\ \hline
Biomarker         & 6                  & $N_{p}*49*6$          & 469134               & 23226                     & 1500                      \\ \hline
\end{tabular}
\caption{Provided datasets statistics across three modalities (OCT, clinical, and biomarker data), where $N_{p}$ indicates the total number of patients}
\label{tab:olives}
\end{table*}

\subsubsection{Open Competition Phase I: Generalization Task}

The overall task in Phase 1 was to predict the presence or absence of six different biomarkers simultaneously on every OCT scan in the provided test set. This task, in general, can be challenging due to different biomarkers exhibiting varying levels of granularity, where some biomarkers are more visually apparent than others. 

The training set for this task was derived from the {\fontfamily{qcr}\selectfont OLIVES} dataset and consisted of the labeled OCT scans, along with the associated clinical information and the corresponding biomarker labels as the ground truth. Participants were encouraged to make use of all available modalities.  Additionally, the participants were provided with a testing dataset that was derived from a recent clinical study in collaboration with Retina Consultants of Texas (Houston, TX, USA). However, teams were only provided with these OCT scans and their clinical information. Thus, participants used all available data to predict the biomarkers associated with each OCT scan in this test set. Once teams had developed their approach, they submitted their algorithms to Codalab for evaluation.

\subsubsection{Open Competition Phase II: Personalization Task}

In Phase 1 of the competition, each slice in the test set was treated as its own independent entity. In reality, however, every set of 49 slices within the test set is associated with a specific patient’s eye. Hence, practitioners may be interested in performance with respect to the patient’s eye as a whole, rather than performance with respect to isolated slices of the retina. Thus, in Phase 2 of the competition the organizers better assess how well the model is able to personalize. 

For Phase 2, the organizers introduce a new held-out test set that replaces the previous test set from the first stage of the competition. This new test set is labeled by our medical partners from Retina Consultants of Texas in the same manner as the first stage, with every image associated with 6 biomarkers. In the Phase 1 test set, a large pool of images are drawn from different visits of the same patient. Hence, Phase 1 test set has substantial redundancy even with a larger number of images, as evidenced by Table~\ref{tab:olives}. Furthermore, the Phase 1 test set was drawn from a clinical trial with similar population demographics to that of the training set. Both of these considerations limit the ability of the original test set to rigorously test the generalizability of the models created in this competition. Hence, the Phase 2 test set is drawn from a larger patient pool and population base which allows a better assessment of both the generalizability and personalization aspects of the submitted algorithms.

Therefore, to perform the personalization aspect of the competition, the registered teams from Phase 1 were given the opportunity to re-train their models and submit the biomarker prediction files for each image in the test set. The overall finalists were then drawn from these performance outcomes on the Phase 2 test set.

\subsection{Resources}

\subsubsection{Datasets and Code}

Teams were provided with access to the labeled {\fontfamily{qcr}\selectfont OLIVES} dataset and another ophthalmology clinical trial dataset from Retina Consultants of Texas for Phase 1, as well as initial Python code using this dataset \cite{prabhushankar2022olives}. In Phase 2, we provide a subset of Kermany dataset for training purposes \cite{kermany2018identifying}. We list a summary of the overall amount of multimodal data included for Phase 1 and Phase 2 in Table \ref{tab:olives}, detailing information about the amount of data included in both train and test sets. The difference in challenge tasks is clearly indicated in this table. For example, in Phase 2, our new held-out test set contained biomarker labels from the Kermany dataset labeled privately by our medical partners \cite{kermany2018identifying}. This difference between Phase 1 and Phase 2 test sets is demonstrated in Table \ref{tab:olives}, where the Phase 2 test set has a much larger patient diversity (167 vs. 40 unique patients) while having fewer images (250 vs. 3871).

% For Phase 1, teams developed their machine learning approaches for biomarker detection using the {\fontfamily{qcr}\selectfont OLIVES} dataset. After teams had developed their respective machine learning approaches, they then submitted their algorithms via Codalab, which evaluated their approach on a held-out test set for biomarker detection indicated in Table \ref{tab:olives}. This held-out test set is from an entirely separate clinical trial, yet it contains the same disease pathology as the provided training set.

% For Phase 2, we introduce a new test set that replaces the previous test set from the first stage of the competition. This new test set is labeled by our medical partners from Retina Consultants of Texas in the same manner as the first stage with every image associated with 6 biomarkers. However, the key difference between the Phase 2 and Phase 1 test set, as shown in Table \ref{tab:olives}, is that the new one has a much larger patient diversity (167 vs. 40 unique patients) while having fewer images (250 vs. 3871). The key problem with the Phase 1 test set is that it had many images, but many of the images were very redundant due to many instances drawn from the same exact patient. Furthermore, the Phase 1 test set was drawn from a clinical trial with similar population demographics to that of the training set. Both of these considerations limit the ability of the original test set to rigorously test the generalizability of the models created in this competition. The Phase 2 test set is drawn from a larger patient pool and population base which allows us to better test the generalizability and thus determine a true winner for the VIP Cup.

\subsubsection{Suggested Methods to Improve Detection}

In addition to starter code, we provide existing works that show improved biomarker detection results. Potential works for improving model performances during detection include, but are not limited to:

\begin{enumerate}
    \item Using multi-modal integration of OCT scans and clinical labels: Clinical labels, such as BCVA and CST, correspond to the health of a patient’s eye, and these clinical values can indicate structural changes within the eye. Therefore, a multi-modal approach to integrate clinical labels via a joint loss may improve accuracy. \cite{prabhushankar2022olives}
    \item Using self-supervised learning with clinical labels: Exploring self-supervised techniques may be an effective way to leverage clinical information for biomarker classification. Since clinical labels can exhibit relationships with biomarkers, \cite{kokilepersaud2022clinical} presents a supervised contrastive loss using clinical labels (BCVA, CST, or a combination of both) for biomarker identification.
    \item Exploiting information about disease severity label: Exploiting information about OCT disease severity may help with biomarker identification, as patients exhibiting similar disease severity levels are more likely to have similar structural characteristics. \cite{kokilepersaud2022gradient} quantifies how anomalous OCT images are relative to a healthy distribution, using this approach to choose pairs for a contrastive learning approach for biomarker classification. Other information that can potentially be leveraged is DRSS, which indicates the severity of the disease. Binning images into similar DRSS scores may also be an approach to understand how anomalous OCT images are.

\end{enumerate}

\subsection{Evaluation Criteria}
We implement two distinct evaluation approaches to judge the teams' generalization and personalization approaches in Phase 1 and 2. The top three teams at the end of Phase 2 are then evaluated to determine the final rankings. In this section, we go over the evaluation criteria for each phase, as well as the criteria the finalists are judged on.

\subsubsection{Phase I Evaluation}

For Phase 1, we draw the test set from an entirely separate clinical trial with the same disease pathology as the training set, where each slice in the test set is treated as its own independent entity in the Phase 1 biomarker detection task. Thus, we make use of the macro averaged F1-score to measure the performance for this phase of the competition. This metric is the equally weighted average of the F1-scores for each of the biomarkers in the 16 biomarker multi-label classification task. There are several characteristics of the dataset that make this metric desirable. The first is that the test set is highly imbalanced, making it impossible to guarantee an equal distribution of biomarkers within each OCT scan. The F1 score is more sensitive to this dataset imbalance, as it is the harmonic mean of precision and recall. In addition, we want our metric to treat each class of biomarker as equally important, rather than reflecting a bias towards classes with more instances present. Therefore, we will designate the top teams as those with the highest macro-averaged F1-score across all 6 biomarkers. With the starter code provided, we achieve a baseline score of 0.6315 when using the described metric for the Phase 1 dataset.

\subsubsection{Phase II Evaluation}

For Phase 2, the test set is from a general population setting and not from a clinical trial. The number of patients are $167$, four times the number in Phase 1 test set. For this portion of the competition, we compute the macro F1-score for each slice in the same way as Phase 1. Unlike Phase 1, however, we will now average the F1-scores with respect to each set of slices associated with an individual patient, rather than averaging across the test set as a whole. This will result in an associated macro F1-score with respect to each individual patient. Teams are ranked with respect to performance on each of the $167$ patients in the test set. Afterwards, the ranking of each team will be averaged across all patients. The three teams with highest performance in Phase 2 are then invited to present their work in the final phase at ICIP 2023. With the provided starter code, we achieve a baseline result of 0.6943 using the described evaluation metric for the Phase 2 data.

\subsubsection{Finalist Judging Criteria}

Judging for the final phase of the competition was held live at the ICIP 2023 conference. It was based on five equally weighted criteria. Each of the three finalist teams are scored on the five criteria and the team with the highest score places 1st, the team with the second highest score places 2nd, and the team with the third highest score places 3rd in the competition. The five equally weighted criteria are: (1) Innovation of the proposed approach, (2) Performance of the team on generalization metric, (3) Performance of the team on personalization metric, (4) Quality and clarity of the final report, and (5) Quality and clarity of the presentation.

Each criterion is scored with a 1, 2, or 3; the best team in each criterion receives 3 points, the second-best team receives 2 points, and the third best team receives 1 point. The final winning rankings are based on the highest points awarded from the five criteria during judge deliberations at the end of the competition. Final rankings are ultimately decided by the judges at their discretion.

==> Sections/5_technical_app.tex <==
%- Need: go through finalists' approaches and document that\\
%- Add: Generalization / personalization graphs from presentation, patient performance ranking, generalization ranking, all F1 scores tables

The finalists for the 2023 VIP CUP Competition are teams Neurons, IITH, and Synapse. In the development of each approach, all teams noted that they had to come to terms with resolving the discrepancy between local and global structures in the provided data. This problem for the associated OCT imaging data is discussed extensively in \cite{kokilepersaud2023clinically} where the authors discuss how algorithms must account for biomarkers with both fine and coarse granularity. The challenge in medical data is that both types of biomarkers can appear simultaneously and models are more likely to identify the easier to identify coarse biomarkers while showing poor performance on the fine-grained biomarkers. We complicate this issue further by having participants consider this problem within the context of both overall generalization as well as within a patient-specific personalization metric. Below, we summarize each approach and specifically highlight, where appropriate, attempts by each team of addressing this granularity issue. Afterwards, we analyze how their differences manifest across performance metrics related to both the personalization and generalization tasks of this competition. 

\paragraph{Team IITH} surprisingly showed that just an Inception v3 \cite{szegedy2015going} backbone with sufficient hyperparameter tuning was enough to obtain competitive performance. The participants arrived at this conclusion after a wide architecture search across a variety of convolutional and transformer based architectures. The team notes that specialized architectural considerations in Inception v3 such as factorizing convolutions, spatially separable convolutions, and efficient grid reduction may enable this architecture to perform feature extraction at multiple scales that is optimal for the biomarker detection task.  
\begin{table*}[]
\centering
\begin{tabular}{cccccccr}
\hline
\multicolumn{8}{|c|}{\textbf{Phase 1 Biomarker-Specific Generalization F1-Score}}                                                                                                                                                                                                             \\ \hline
\multicolumn{1}{|c|}{\textbf{Team}} & \multicolumn{1}{c|}{\textbf{B1}} & \multicolumn{1}{c|}{\textbf{B2}} & \multicolumn{1}{c|}{\textbf{B3}} & \multicolumn{1}{c|}{\textbf{B4}} & \multicolumn{1}{c|}{\textbf{B5}} & \multicolumn{1}{c|}{\textbf{B6}} & \multicolumn{1}{c|}{\textbf{Overall}} \\ \hline
Elemenopi                           & 0.656                            & 0.756                            & 0.784                            & 0.832                            & 0.852                            & \textbf{0.992}                   & 0.7518                                \\
IITH                                & 0.684                            & 0.74                             & 0.732                            & 0.94                             & 0.864                            & \textbf{0.992}                   & 0.747                                 \\
MEA                                 & 0.38                             & 0.62                             & 0.592                            & 0.636                            & 0.156                            & 0.02                             & 0.197                                 \\
Neurons                             & 0.648                            & 0.76                             & 0.788                            & 0.96                             & 0.768                            & 0.984                            & 0.779                                 \\
Optimpus                            & 0.688                            & 0.488                            & 0.512                            & 0.776                            & 0.852                            & \textbf{0.992}                   & 0.646                                 \\
Pixel Pulse                         & 0.652                            & 0.664                            & 0.656                            & 0.912                            & 0.788                            & 0.564                            & 0.532                                 \\
Pixel Vision                        & 0.476                            & 0.648                            & 0.6                              & 0.648                            & 0.16                             & 0.072                            & 0.398                                 \\
Sharks                              & 0.652                            & 0.696                            & 0.632                            & 0.616                            & 0.848                            & \textbf{0.992}                   & 0.668                                 \\
Source Code                         & 0.676                            & 0.552                            & 0.492                            & 0.848                            & \textbf{0.884}                   & 0.916                            & 0.6133                                \\
Spectrum                            & 0.716                            & 0.74                             & 0.748                            & 0.908                            & 0.804                            & 0.968                            & 0.7504                                \\
Synapse                             & 0.712                            & \textbf{0.776}                   & \textbf{0.836}                   & \textbf{0.956}                   & 0.86                             & \textbf{0.992}                   & \textbf{0.806}                        \\
Tesseract                           & 0.732                            & 0.676                            & 0.592                            & 0.932                            & 0.848                            & \textbf{0.992}                   & 0.644                                 \\
Ultrabot AIO                        & 0.732                            & 0.632                            & 0.604                            & 0.92                             & 0.856                            & 0.976                            & 0.721                                 \\
UNNC\_ISEAN                         & \textbf{0.76}                    & 0.74                             & 0.776                            & 0.136                            & 0.82                             & 0.132                            & 0.568                                 \\
UNNC\_POWER                         & 0.72                             & 0.728                            & 0.756                            & 0.536                            & \textbf{0.884}                   & 0.036                            & 0.543                                 \\ \hline
\multicolumn{8}{|c|}{\textbf{Phase 2 Biomarker-Specific Personalization F1-Score}}                                                                                                                                                                                                            \\ \hline
\multicolumn{1}{|c|}{\textbf{Team}} & \multicolumn{1}{c|}{\textbf{B1}} & \multicolumn{1}{c|}{\textbf{B2}} & \multicolumn{1}{c|}{\textbf{B3}} & \multicolumn{1}{c|}{\textbf{B4}} & \multicolumn{1}{c|}{\textbf{B5}} & \multicolumn{1}{c|}{\textbf{B6}} & \multicolumn{1}{c|}{\textbf{Overall}} \\ \hline
\textbf{IITH}                       & 0.6893                           & 0.7528                           & 0.7578                           & 0.9483                           & \textbf{0.8516}                  & \textbf{0.988}                   & \textbf{0.8215}                       \\
\textbf{Neurons}                    & 0.6397                           & 0.7762                           & 0.7891                           & \textbf{0.9657}                  & 0.7684                           & 0.9847                           & \textbf{0.8116}                       \\
\textbf{Synapse}                    & 0.7173                           & \textbf{0.7946}                  & \textbf{0.8525}                  & 0.9632                           & 0.8456                           & \textbf{0.988}                   & \textbf{0.8527}                       \\
\hline
Elemenopi                           & 0.6527                           & 0.7734                           & 0.8122                           & 0.817                            & 0.8396                           & \textbf{0.988}                   & 0.7966                                \\
MEA                                 & 0.3861                           & 0.6236                           & 0.592                            & 0.636                            & 0.172                            & 0.0299                           & 0.3822                                \\
Optimpus                            & 0.6897                           & 0.5087                           & 0.5207                           & 0.7902                           & 0.8506                           & 0.988                            & 0.697                                 \\
Pixel Pulse                         & 0.6477                           & 0.6709                           & 0.6954                           & 0.9183                           & 0.7926                           & 0.556                            & 0.6984                                \\
Pixel Vision                        & 0.4774                           & 0.6466                           & 0.6188                           & 0.6903                           & 0.1727                           & 0.0689                           & 0.4139                                \\
Sharks                              & 0.647                            & 0.6889                           & 0.6282                           & 0.6191                           & 0.8306                           & \textbf{0.988}                   & 0.7056                                \\
Source Code                         & 0.7028                           & 0.587                            & 0.4977                           & 0.8627                           & 0.8849                           & 0.9254                           & 0.7274                                \\
Spectrum                            & 0.7326                           & 0.7518                           & 0.7505                           & 0.9068                           & 0.8038                           & 0.9676                           & 0.8067                                \\
Tesseract                           & 0.744                            & 0.6928                           & 0.6158                           & 0.9378                           & 0.8336                           & \textbf{0.988}                   & 0.7921                                \\
Ultrabot AIO                        & 0.7421                           & 0.6364                           & 0.5963                           & 0.9311                           & 0.8425                           & 0.9757                           & 0.7723                                \\
UNNC\_ISEAN                         & \textbf{0.771}                   & 0.7658                           & 0.7997                           & 0.1379                           & 0.8086                           & 0.1349                           & 0.5426                                \\
UNNC\_POWER                         & 0.7178                           & 0.7464                           & 0.7897                           & 0.5241                           & 0.8739                           & 0.0479                           & 0.593                                
\end{tabular}
\caption{The F1-Scores for all 15 teams on individual biomarkers across both phases of the competition are shown above. For Phase 2, the final three teams (IITH, Neurons, and Synapse) are bolded.}
\label{tab:biomarker}
\end{table*}
% \begin{table*}[]
% \centering

% \begin{tabular}{@{}lcccccc@{}}
% \toprule
% \multicolumn{7}{c}{Phase 1 Biomarker-Specific Generalization F1-Score}                                                                                        \\ \midrule
% Team    & \multicolumn{1}{l}{B1} & \multicolumn{1}{l}{B2} & \multicolumn{1}{l}{B3} & \multicolumn{1}{l}{B4} & \multicolumn{1}{l}{B5} & \multicolumn{1}{l}{B6} \\ \midrule
% Neurons & 0.648                  & 0.760                  & 0.788                  & \textbf{0.960}         & 0.768                  & 0.984                  \\
% IITH    & 0.684                  & 0.740                  & 0.732                  & 0.940                  & \textbf{0.864}         & \textbf{0.992}         \\
% Synapse & \textbf{0.712}         & \textbf{0.776}         & \textbf{0.836}         & 0.956                  & 0.860                  & \textbf{0.992}         \\ \midrule
% \multicolumn{7}{c}{Phase 2 Biomarker-Specific Personalization F1-Score}                                                                                       \\ \midrule
% Team    & \multicolumn{1}{l}{B1} & \multicolumn{1}{l}{B2} & \multicolumn{1}{l}{B3} & \multicolumn{1}{l}{B4} & \multicolumn{1}{l}{B5} & \multicolumn{1}{l}{B6} \\ \midrule
% Neurons & 0.639                  & 0.776                  & 0.789                  & \textbf{0.965}         & 0.768                  & 0.9847                 \\
% IITH    & 0.689                  & 0.752                  & 0.757                  & 0.948                  & \textbf{0.851}         & \textbf{0.988}         \\
% Synapse & \textbf{0.717}         & \textbf{0.794}         & \textbf{0.852}         & 0.963                  & 0.845                  & \textbf{0.988}         \\ \bottomrule
% \end{tabular}
% \label{tab:biomarker}
% \caption{The F1-Scores for the top 3 teams on individual biomarkers across both phases of the compeititon are shown above.}
% \end{table*}

\paragraph{Team Neurons} made the insight that convolutional networks (CNN) are good at local feature extraction with their fixed kernels, while transformers use attention to extract features from a global context. Therefore, using an ensemble of both enables extraction of both types of features. Specifically, the used an EfficientNet \cite{tan2019efficientnet} architecture for local feature extraction and a Max-ViT \cite{tu2022maxvit} transformer  for global understanding. They then split the overall OLIVES dataset based on TREX or PRIME clinical trials specifically. The ensemble was then formed by training their models on the subsets TREX + PRIME, TREX only, and PRIME only. This allows different subsets of the models to be tuned to the different types of features that each trial provides. During inference, each pair of models trained on each subset to produce a prediction that are then used in an ensemble fashion to produce the final decision.

\paragraph{Team Synapse} made the observation that an ensemble of models with one performing local feature extraction and one performing global attention is optimal for this task due to biomarkers of varying granularity. However, in contrast to team Neurons, they used a vision transformer with a convolutional block as the local feature extractor, rather than a CNN alone. In this case, Max-VIT \cite{tu2022maxvit} was the local extractor and EVA-02 \cite{fang2023eva} performed global attention. The team notes that the the use of normal attention compared to strided attention causes the global vs. local feature extraction capability. An ensemble was then created by having Max-VIT predict only fine-grained biomarkers, while EVA-02 was responsible for coarse-grained biomarkers.

A closer look at the performance of each approach in a variety of settings provides deeper insight into the personalization and generalization capabilities of each algorithm. In Table \ref{tab:biomarker}, we note the performance of all teams on individual biomarkers. When analyzing the three finalists' results, we observe that all teams performed similarly well on B4, B5, and B6, but a substantial gap exists on B1, B2, and B3. Team Synapse performed better on the more difficult fine-grained biomarkers compared to either of the other two finalists. This trend holds for both the personalization and generalization performance and suggests that their approach was able to rectify local and global features to a greater extent. 


\begin{figure}[h]
\centerline{\includegraphics[scale=.53]{Images/Performance_Graphs/biomarker_team_rankings.jpg}}
\caption{This figure shows the average and associated standard deviation of the ranking of each team on each biomarker with first being the best. The top three teams overall are highlighted in red.}
\label{biomarker_ranking}
\end{figure}

\begin{figure}[h]
\centerline{\includegraphics[scale=.53]{Images/Performance_Graphs/patient_good_performance.jpg}}
\caption{This shows the number of patients on the test set where the performance exceeded a good F1-Score threshold (.8) for each team in the competition. The top 3 teams are highlighted in red.}
\label{patients_ranking}
\end{figure}

\begin{figure}[h]
\centerline{\includegraphics[scale=.55]{Images/Performance_Graphs/Phase_1_2_performance_correlate.jpg}}
\caption{This plot shows the correlation shows every team's generalization and personalization performance.}
\label{generalization_personalization}
\end{figure}

\begin{figure}[h]
\centerline{\includegraphics[scale=.55]{Images/Performance_Graphs/Patient_2_performance_correlate.jpg}}
\caption{This plot shows how well every team's personalization performance correlates with the number of patients that have a good (.8 or higher) associated F1-Score.}
\label{personal_ranking}
\end{figure}

We also ranked each team from 1 to 16 in Figure \ref{biomarker_ranking} based on their generalization performance on each biomarker and analyzed the average ranking across all teams. Team Synapse and IITH performed consistently well across all biomarkers. Team Neurons exhibited higher variation as shown by better performance on specific biomarkers, but worse on others. We also ranked teams based on the number of patients where performance crossed a satisfactory F1-score threshold (0.8). All the top-performing teams had the most number of patients where their performance was above this threshold as shown in Figure \ref{patients_ranking}. 

In Figures \ref{generalization_personalization} we show a scatter plot that demonstrates how correlated performance on the generalization and personalization tasks are for each team. Overall, it seems that doing well on one task transfers to doing well on the other. Additionally, we observe that personalization performance correlates with performing well on a higher number of patients as shown in Figure \ref{personal_ranking}. In both plots, the top 3 teams clustered in the high performing top-right region of the figures. Additionally, this comes with a noticeable separation from the overall winner Team Synapse. 



==> Sections/6_feedback.tex <==
In this section, we discuss insights used to create the VIP Cup 2023 challenge and the issues faced throughout the competition. From an organization standpoint, the topic of integrating artificial intelligence (AI) within medicine is one that has gained much attention within the research community within recent years and presents an excellent avenue towards introducing students to real-world applications of artificial intelligence. Ophthalmology, in particular, has been described as the first clinical application domain that has the potential for full automation \cite{beede2020human}. This is primarily because OCT and fundus photography are oftentimes easier to derive features from due to easier noise characteristics compared to other modalities of medical imaging tasks, making this type of data more amenable to AI algorithms that rely on deriving standard features to distinguish different classes. This is demonstrated in Figure \ref{data}, where the structures present in OCT are clearly visible, as opposed to the images taken from a dermatology (DermMNIST) and chest x-ray dataset (PadChest) \cite{yang2023medmnist}, \cite{bustos2020padchest}.

\begin{figure}[h]
\centerline{\includegraphics[width=0.45\textwidth]{Images/datasets.png}}
\caption{Difference in noise characteristics between OCT, dermatology, and chest x-ray images}
\label{data}
\end{figure}

Another advantage of using OCT data is that it is associated with a clinical trial structure, rather than as isolated instances~\cite{fowler2023clinical}. The clinical trial structure enables the existence of many different modalities such as textual documents, clinical values, and other imaging modalities~\cite{logan2022decal}. Therefore, students get exposure to the existence and interaction of these different axes within the medical domain. Furthermore, the clinical trial structure acts as a regularizer in terms of the scope of the data they have access to. In other words, the size of the data they have access to is limited by the resources of the clinical trial thus preventing the existence of too large of a data source for students to work with effectively. This is important within the context of the VIP Cup such that the competition is accessible to students from different regions and backgrounds who may have lesser access to computational sources than others. Additionally, the clinical trial structure ensures that data is composed from wider demographic sources, which in turn ensures that the solutions devised by the students is indeed generalizable.

%Another major aspect is to get students used to the idea of handling data and performing some type of preprocessing pipeline before training models. OCT data is useful for this task because students have to consider whether some noise-reduction or edge enhancement strategy is useful before engaging in complete training.

We now discuss the competition from an organization standpoint, as observed by the organizing committee (Figure \ref{olives-team}). When running the VIP Cup competition, we initially utilized Codalab for our project needs, which had automatic migration of Phase 1 submissions for hidden Phase 2 evaluations. However, we encountered performance and accessibility issues. Due to the high volume of traffic and migration of submissions on the Codalab platform, the server crashed. To combat this problem, we established a mirror site, where the submission resulted in a direct scoring without need for migration. This change drastically improved performance and reliability. Submissions were seamless with faster scoring, proving that the establishment of the mirror site was an efficient solution. This observation was corroborated by participating teams, as one team noted that for future VIP Cup iterations a more mature platform might be a better solution. Despite this issue, Team Synapse notes the following for the VIP Cup challenge: "All in all, VIP Cup 2023 was a monumental experience for our team, and thanks once again." 
%participating teams noted that the VIP Cup challenge was monumental, serving as a fun and educational experience to those involved.
% \begin{figure}
% \centerline{\includegraphics[scale=.058]{Images/olives_pic.jpg}}
% \caption*{Organizing committee from the Olives lab at Georgia Institute of Technology. From left to right: Kiran Kokilepersaud, Prithwijit Chowdhury, Zoe Fowler, Ghassan AlRegib, and Mohit Prabhushankar.}
% \label{olives-team}
% \end{figure}
